Perception Stitching: Zero-Shot Perception Encoder Transfer for Visuomotor Robot Policies

Vision-based imitation learning has shown promising capabilities of endowing robots with various motion skills given visual observation. However, current visuomotor policies fail to adapt to drastic changes in their visual observations. We present Perception Stitching that enables strong zero-shot adaptation to large visual changes by directly stitching novel combinations of visual encoders. Our key idea is to enforce modularity of visual encoders by aligning the latent visual features among different visuomotor policies. Our method disentangles the perceptual knowledge with the downstream motion skills and allows the reuse of the visual encoders by directly stitching them to a policy network trained with partially different visual conditions. We evaluate our method in various simulated and real-world manipulation tasks. While baseline methods failed at all attempts, our method could achieve zero-shot success in real-world visuomotor tasks. Our quantitative and qualitative analysis of the learned features of the policy network provides more insights into the high performance of our proposed method.

==> tables/qa_anchors_from_failure_zero_shot.tex <==
\begin{table*}[!ht]
\centering
\begin{tabular}{l|cccccc|c}
\toprule
 & Mask & Zoom in & Blurred & Noise & Fisheye & Camera Position & Average \\
\midrule
100\% success rate & 94.7$\pm$0.94 & \textbf{96.7$\pm$0.94} & \textbf{90.0$\pm$1.63} & 96.7$\pm$1.89 & \textbf{97.3$\pm$2.49} & 80.0$\pm$4.90 & \textbf{92.6} \\
54\% success rate & \textbf{98.7$\pm$0.94} & 95.3$\pm$3.77 & 46.0$\pm$1.63 & 85.3$\pm$0.94 & 52.7$\pm$2.49 & 84.0$\pm$3.27 & 77.0 \\
6\% success rate & 49.3$\pm$6.80 & 48.7$\pm$4.11 & 76.7$\pm$8.06 & \textbf{98.7$\pm$0.94} & 44.7$\pm$3.40 & \textbf{98.0$\pm$1.63} & 69.4 \\
\bottomrule
\end{tabular}
\caption*{\textbf{Table C: Anchors from Failure Trajectories.} All the experiments are carried out with the Stack task. We chose anchor datasets from three different datasets with K-means algorithm: (1) The dataset is collected by an expert agent, and it contains $200$ success trajectories. (2) The dataset is collected by an semi-trained policy which has around 50\% of success rate. It is used to collect 200 trajectories, among which 54\% are successful trajectories and 46\% are failure trajectories. (3) The dataset is collected by a poorly behaved policy with a close to zero success rate. It is used to collect 200 trajectories, among which only 6\% are successful trajectories and 94\% are failure trajectories. The average success rate decreases when the percentage of successful trajectories in the dataset for anchor selection decreases.}
\label{tab:anchor_sr}
\end{table*}


==> tables/qa_decoder1_vs_decoder2.tex <==
\begin{table*}[!ht]
\centering
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{c|c|cccccc|c}
\toprule
 &  & \textbf{Mask} & \textbf{Zoom in} & \textbf{Blurred} & \textbf{Noise} & \textbf{Fisheye} & \textbf{Camera Position} & \textbf{Average} \\
\midrule
\multicolumn{1}{c|}{\multirow{2}{*}{Devin et al. 2017}} & Decoder 1                    & 0.7$\pm$0.94 & \textbf{8.0$\pm$1.63} & 0.7$\pm$0.94 & \textbf{24.0$\pm$2.83} & 0.0$\pm$0.00 & \textbf{14.0$\pm$3.27} & \textbf{7.9}    \\

\multicolumn{1}{c|}{}                     & Decoder 2               &\textbf{5.3$\pm$2.49} & 0.0$\pm$0.00 & \textbf{14.0$\pm$2.83} & 6.7$\pm$2.49 & \textbf{3.3$\pm$1.89} & 5.3$\pm$2.49 & 5.8    \\ \hline

\multicolumn{1}{c|}{\multirow{2}{*}{Cannistraci et al. 2024 (linear)}} & Decoder 1                    & \textbf{47.3$\pm$0.94} & \textbf{62.0$\pm$4.32} & \textbf{32.7$\pm$3.77} & 30.7$\pm$0.94 & \textbf{54.0$\pm$8.64} & 14.7$\pm$6.18 & 40.2    \\

\multicolumn{1}{c|}{}                     & Decoder 2               & 39.3$\pm$4.11 & 56.7$\pm$1.89 & 26.7$\pm$6.60 & \textbf{51.3$\pm$4.11} & 46.0$\pm$2.83 & \textbf{23.3$\pm$1.89} & \textbf{40.6}    \\ \hline

\multicolumn{1}{c|}{\multirow{2}{*}{Cannistraci et al. 2024 (non-linear)}} & Decoder 1                    & \textbf{10.0$\pm$1.63} & \textbf{12.0$\pm$0.00} & 0.0$\pm$0.00 & 3.3$\pm$0.94 & 0.0$\pm$0.00 & \textbf{0.7$\pm$0.94} & 4.3    \\ 

\multicolumn{1}{c|}{}                     &  Decoder 2 & 5.3$\pm$0.94 & 6.7$\pm$0.94 & \textbf{8.0$\pm$2.83} & \textbf{14.7$\pm$1.89} & \textbf{2.0$\pm$1.63} & 0.0$\pm$0.00 & \textbf{6.1}    \\ \hline

\multicolumn{1}{c|}{\multirow{2}{*}{PeS (-w/o disent. loss)}} & Decoder 1                    & \textbf{34.0$\pm$11.43} & 10.7$\pm$4.11 & \textbf{62.0$\pm$10.71} & \textbf{34.0$\pm$7.12} & 22.7$\pm$3.77 & \textbf{26.0$\pm$4.32} & 31.6    \\

\multicolumn{1}{c|}{}                     & Decoder 2               &31.3$\pm$2.49 & \textbf{52.7$\pm$6.60} & 28.0$\pm$3.27 & 26.7$\pm$1.89 & \textbf{32.7$\pm$3.40} & 19.3$\pm$4.11 & \textbf{31.8}    \\ \hline

\multicolumn{1}{c|}{\multirow{2}{*}{PeS (w. l1 \& l2 loss)}} & Decoder 1                    & \textbf{92.7$\pm$0.94} & \textbf{98.0$\pm$0.00} & 62.7$\pm$6.60 & 24.0$\pm$4.90 & \textbf{59.3$\pm$7.36} & \textbf{58.7$\pm$1.88} & \textbf{65.9}    \\

\multicolumn{1}{c|}{}                     & Decoder 2               & 72.7$\pm$3.77 & 36.0$\pm$1.63 & \textbf{88.7$\pm$4.99} & \textbf{58.7$\pm$1.88} & 23.3$\pm$3.40 & 33.3$\pm$0.94 & 52.1    \\ \hline

\multicolumn{1}{c|}{\multirow{2}{*}{PeS}} & Decoder 1                    & \textbf{94.7$\pm$0.94} & \textbf{96.7$\pm$0.94} & 90.0$\pm$1.63 & \textbf{96.7$\pm$1.89} & \textbf{97.3$\pm$2.49} & \textbf{80.0$\pm$4.90} & \textbf{92.6}    \\ 

\multicolumn{1}{c|}{}                     &  Decoder 2 & 83.3$\pm$4.11 & 86.0$\pm$4.32 & \textbf{94.0$\pm$2.83} & 92.7$\pm$0.94 & 95.3$\pm$0.94 & 68.7$\pm$6.18 & 85.0    \\
\bottomrule
\end{tabular}
}
\caption*{\textbf{Table D: Action Decoder 1 V.S. Action Decoder 2.} All the experiments are carried out with the Stack task. For the PeS method and other baseline and ablation methods, the difference in the average success rates of using action decoder 1 or action decoder 2 is within 15\%. The choice of the action decoder does not have any distinct influence on the zero-shot transfer success rates.}
\label{tab:decoder1_vs_decoder2}
\vspace{-10pt}
\end{table*}







==> tables/qa_one_black_image_zero_shot.tex <==
\begin{table*}[!ht]
\centering
\begin{tabular}{l|ccccc|c}
\toprule
 & Push & Lift & Can & Stack & Door Open & Average \\
\midrule
Devin et al. 2017 & 73.3$\pm$11.47 & 72.7$\pm$0.94 & 66.7$\pm$6.18 & 14.0$\pm$3.27 & 22.7$\pm$2.50 & 49.8 \\
Cannistraci et al. 2024 (linear) & 89.3$\pm$4.11 & 86.0$\pm$1.63 & 72.8$\pm$3.27 & 14.7$\pm$6.18 & 39.3$\pm$3.40 & 60.4 \\
Cannistraci et al. 2024 (non-linear) & 60.7$\pm$1.88 & 80.7$\pm$3.40 & 24.0$\pm$2.83 & 0.7$\pm$0.94 & 41.3$\pm$4.99 & 41.5 \\
PeS (-w/o disent. loss) & 88.7$\pm$4.11 & \textbf{94.0$\pm$1.63} & 91.0$\pm$3.40 & 26.0$\pm$4.32 & 32.7$\pm$3.77 & 66.5 \\
PeS (w. l1 \& l2 loss) & \textbf{94.7$\pm$2.49} & 90.0$\pm$2.83 & 86.7$\pm$1.89 & 58.7$\pm$1.88 & 40.7$\pm$0.94 & 74.2 \\
PeS & 91.3$\pm$2.49 & 92.6$\pm$0.94 & \textbf{94.6$\pm$0.94} & \textbf{80.0$\pm$4.90} & \textbf{72.7$\pm$3.77} & \textbf{86.2} \\
\bottomrule
\end{tabular}%
\caption*{\textbf{Table A: Zero-Shot Transfer Success Rates of single camera policies.} PeS achieves optimal performance in the three difficult tasks (Can, Stack, Door Open), and close-to optimal performance in the two basic tasks (Push, Lift). Its average success rate outperforms all the baselines and the ablation methods.}
\label{tab:qa_black_img_stitch}
\end{table*}


==> tables/qa_sim_zero_shot_hard.tex <==
\begin{table*}[!ht]
\centering
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{c|c|cccccc|c}
\toprule
 &  & \textbf{Mask} & \textbf{Zoom in} & \textbf{Blurred} & \textbf{Noise} & \textbf{Fisheye} & \textbf{Camera Position} & \textbf{Average} \\
\midrule
\multicolumn{1}{c|}{\multirow{6}{*}{Can}} & Devin et al. 2017                    & 19.3$\pm$5.25 & 24.7$\pm$1.89 & 2.67$\pm$1.89 & 6.0$\pm$4.32 & 29.3$\pm$3.40 & 1.3$\pm$1.89 & 13.9    \\

\multicolumn{1}{c|}{}                     & Cannistraci et al. 2024 (linear)     & 33.3$\pm$0.94 & 48.0$\pm$1.63 & 48.7$\pm$2.49 & 65.3$\pm$0.94 & 26.7$\pm$3.77 & 34.7$\pm$3.77 & 42.8    \\ 

\multicolumn{1}{c|}{}                     & Cannistraci et al. 2024 (non-linear) & 72.7$\pm$0.94 & 24.7$\pm$2.49 & 37.3$\pm$4.99 & 42.7$\pm$3.40 & 8.7$\pm$1.89 & 39.3$\pm$1.89 & 37.6    \\ 

\multicolumn{1}{c|}{}                     & PeS (w/o disent. loss)               & 44.7$\pm$8.06 & \textbf{89.3$\pm$4.11} & 34.7$\pm$4.11 & 30.7$\pm$6.80 & \textbf{92.7$\pm$2.50} & 44.7$\pm$3.40 & 56.1    \\ 

\multicolumn{1}{c|}{}                     & PeS (w. l1 \& l2 loss)               & 47.3$\pm$0.94 & 58.7$\pm$1.88 & 54.0$\pm$8.64 & 36.0$\pm$7.12 & 58.7$\pm$1.88 & 64.7$\pm$6.60 & 53.2    \\
\multicolumn{1}{c|}{}                     & PeS               &\textbf{83.3$\pm$5.24} & \textbf{89.3$\pm$2.49} & \textbf{74.0$\pm$2.83} & \textbf{78.7$\pm$4.11} & 56.0$\pm$2.83 & \textbf{78.7$\pm$2.49} & \textbf{76.7}    \\ \hline

\multicolumn{1}{c|}{\multirow{6}{*}{Stack}} & Devin et al. 2017                    & 0.7$\pm$0.94 & 8.0$\pm$1.63 & 0.7$\pm$0.94 & 24.0$\pm$2.83 & 0.0$\pm$0.00 & 14.0$\pm$3.27 & 7.9    \\

\multicolumn{1}{c|}{}                     & Cannistraci et al. 2024 (linear)     & 47.3$\pm$0.94 & 62.0$\pm$4.32 & 32.7$\pm$3.77 & 30.7$\pm$0.94 & 54.0$\pm$8.64 & 14.7$\pm$6.18 & 40.2    \\ 

\multicolumn{1}{c|}{}                     & Cannistraci et al. 2024 (non-linear) & 10.0$\pm$1.63 & 12.0$\pm$0.00 & 0.0$\pm$0.00 & 3.3$\pm$0.94 & 0.0$\pm$0.00 & 0.7$\pm$0.94 & 4.3    \\ 

\multicolumn{1}{c|}{}                     & PeS (w/o disent. loss)               & 34.0$\pm$11.43 & 10.7$\pm$4.11 & 62.0$\pm$10.71 & 34.0$\pm$7.12 & 22.7$\pm$3.77 & 26.0$\pm$4.32 & 31.6    \\ 

\multicolumn{1}{c|}{}                     & PeS (w. l1 \& l2 loss)               & 92.7$\pm$0.94 & \textbf{98.0$\pm$0.00} & 62.7$\pm$6.60 & 24.0$\pm$4.90 & 59.3$\pm$7.36 & 58.7$\pm$1.88 & 65.9    \\
\multicolumn{1}{c|}{}                     & PeS               & \textbf{94.7$\pm$0.94} & 96.7$\pm$0.94 & \textbf{90.0$\pm$1.63} & \textbf{96.7$\pm$1.89} & \textbf{97.3$\pm$2.49} & \textbf{80.0$\pm$4.90} & \textbf{92.6}    \\ \hline

\multicolumn{1}{c|}{\multirow{6}{*}{Door\ Open}} & Devin et al. 2017                    & 9.3$\pm$4.11 & 5.3$\pm$0.94 & 0.0$\pm$0.00 & 4.0$\pm$1.63 & 0.7$\pm$0.94 & 0.0$\pm$0.00 & 3.2    \\ 

\multicolumn{1}{c|}{}                     & Cannistraci et al. 2024 (linear)     & 0.0$\pm$0.00 & 1.3$\pm$0.94 & 10.7$\pm$2.49 & 10.7$\pm$4.99 & 2.0$\pm$1.63 & 47.3$\pm$9.29 & 12    \\ 

\multicolumn{1}{c|}{}                     & Cannistraci et al. 2024 (non-linear) & 26.0$\pm$2.83 & 31.3$\pm$4.99 & 49.3$\pm$8.22 & 48.0$\pm$5.89 & 62.7$\pm$3.40 & 44.7$\pm$3.40 & 43.7    \\ 

\multicolumn{1}{c|}{}                     & PeS (w/o disent. loss)               & 24.7$\pm$7.71 & 44.0$\pm$2.83 & 34.7$\pm$3.77 & 0.7$\pm$0.94 & 36.7$\pm$0.94 & 23.3$\pm$3.40 & 27.4    \\ 

\multicolumn{1}{c|}{}                     & PeS (w. l1 \& l2 loss)               & 4.0$\pm$1.63 & \textbf{78.0$\pm$5.66} & 3.3$\pm$0.94 & 2.0$\pm$1.63 & 42.7$\pm$4.99 & 6.0$\pm$3.26 & 22.7    \\

\multicolumn{1}{c|}{}                     &  PeS & \textbf{58.7$\pm$4.11} & 68.7$\pm$0.94 & \textbf{70.7$\pm$0.94} & \textbf{52.7$\pm$3.40} & \textbf{64.7$\pm$4.99} & \textbf{48.7$\pm$3.40} & \textbf{60.7}    \\
\bottomrule
\end{tabular}
}
\caption*{\textbf{Table E: Zero-Shot Transfer Success Rates in difficult Simulation tasks.} The three difficult tasks include Can, Stack, and Door Open. We test all methods across six different visual configurations and also calculate the average performance. The three baselines achieve about 0\% - 40\% of success rates in these tasks. In the Can and Stack tasks, PeS achieves 75\% - 95\% of success rates, while the ablation methods achieves about 30\% - 65\% of success rates. In the Door task, PeS achieves 60.7\% of success rates, while the two ablation methods only have 20\% - 30\% of success rates.}
\label{tab:sim_zero_shot_hard}
\end{table*}







==> tables/qa_three_cameras_zero_shot.tex <==
\begin{table*}[!ht]
\centering
\begin{tabular}{l|cccccc|c}
\toprule
 & Mask & Zoom in & Blurred & Noise & Fisheye & Camera Position & Average \\
\midrule
Devin et al. 2017 & 4.0$\pm$1.63 & 5.3$\pm$2.49 & 1.3$\pm$0.94 & 13.3$\pm$1.89 & 1.3$\pm$1.89 & 8.0$\pm$1.63 & 5.5 \\

Cannistraci et al. 2024 (linear) & 46.7$\pm$3.40 & 20.7$\pm$1.89 & 13.3$\pm$1.89 & 56.0$\pm$2.83 & 16.0$\pm$4.32 & 30.0$\pm$4.32 & 30.5 \\

Cannistraci et al. 2024 (non-linear) & 30.7$\pm$0.94 & 22.7$\pm$0.94 & 19.3$\pm$4.11 & 42.7$\pm$1.89 & 12.7$\pm$0.94 & 4.7$\pm$2.49 & 22.1 \\

PeS (-w/o disent. loss) & 21.3$\pm$2.49 & 20.7$\pm$1.89 & 72.7$\pm$3.77 & 56.7$\pm$4.11 & 37.3$\pm$4.99 & 9.3$\pm$1.89 & 36.3 \\

PeS (w. l1 \& l2 loss) & 46.7$\pm$3.40 & 56.7$\pm$4.11 & 84.0$\pm$2.83 & 82.7$\pm$2.49 & 75.3$\pm$2.49 & 61.3$\pm$3.40 & 67.8 \\

PeS & \textbf{97.3$\pm$2.49} & \textbf{92.7$\pm$0.94} & \textbf{93.3$\pm$0.94} & \textbf{90.0$\pm$1.63} & \textbf{94.6$\pm$0.94} & \textbf{86.7$\pm$2.49} & \textbf{92.4} \\

\bottomrule
\end{tabular}%
\caption*{\textbf{Table B: Zero-Shot Transfer Success Rates of triple camera policies.} All the experiments are carried out with the Stack task. PeS achieves optimal performance for all the six different visual configurations. Its average success rate has an around 25\% advantage to the second best method.}
\label{tab:three_cameras_stitch}
\end{table*}


==> tables/sim_zero_shot.tex <==
% \begin{table*}[!ht]
%   \centering
%   \begin{tabular}{lcccccccc}
%     \toprule % Top horizontal line
%     & \multicolumn{2}{c}{Push} & \multicolumn{2}{c}{Lift} & \multicolumn{2}{c}{Can} & \multicolumn{2}{c}{Stack} \\
%     \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} % Partial horizontal lines under the subheadings
%     & ours & baseline & ours & baseline & ours & baseline & ours & baseline \\
%     \midrule % Middle horizontal line
%     Masked & \textbf{100.0 $\pm$ 0.00} & 60.7 $\pm$ 10.6 & \textbf{83.3 $\pm$ 6.60} & 0.0 $\pm$ 0.00 & \textbf{44.7 $\pm$ 8.06} & 19.3 $\pm$ 5.25 & \textbf{34.0 $\pm$ 11.43} & 0.7 $\pm$ 0.94 \\
%     Zoom in & \textbf{86.0 $\pm$ 2.83} & 8.7 $\pm$ 4.99 & \textbf{80.7 $\pm$ 5.73} & 5.3 $\pm$ 2.49 & \textbf{89.3 $\pm$ 4.11} & 24.7 $\pm$ 1.89 & \textbf{10.7 $\pm$ 4.11} & 8.0 $\pm$ 1.63 \\
%     Blurred & \textbf{80.7 $\pm$ 9.84} & 16.7 $\pm$ 3.77 & \textbf{93.3 $\pm$ 0.94} & 48.0 $\pm$ 5.89 & \textbf{34.7 $\pm$ 4.11} & 2.67 $\pm$ 1.89 & \textbf{62.0 $\pm$ 10.71} & 0.7 $\pm$ 0.94 \\
%     Gaussian Noise & \textbf{100.0 $\pm$ 0.00} & 59.3 $\pm$ 6.80 & \textbf{91.3 $\pm$ 5.73} & 9.3 $\pm$ 4.11 & \textbf{30.7 $\pm$ 6.80} & 6.0 $\pm$ 4.32 & \textbf{34.0 $\pm$ 7.12} & 24.0 $\pm$ 2.83 \\
%     Camera Type & \textbf{100.0 $\pm$ 0.00} & 29.3 $\pm$ 7.36 & \textbf{79.3 $\pm$ 2.49} & 14.7 $\pm$ 4.99 & \textbf{92.7 $\pm$ 2.50} & 29.3 $\pm$ 3.40 & \textbf{22.7 $\pm$ 3.77} & 0.0 $\pm$ 0.00 \\
%     Camera Position & \textbf{100.0 $\pm$ 0.00} & 19.3 $\pm$ 5.73 & \textbf{93.3 $\pm$ 2.49} & 36.0 $\pm$ 1.63 & \textbf{44.7 $\pm$ 3.40} & 1.3 $\pm$ 1.89 & \textbf{26.0 $\pm$ 4.32} & 14.0 $\pm$ 3.27 \\
%     \bottomrule % Bottom horizontal line
%   \end{tabular}
%   \caption{Zero shot transfer results in simulation.}
%   \label{tab:sim_zero_shot}
% \end{table*}



\begin{table*}[!ht]
  \centering
  \begin{tabular}{@{} l *{8}{c} @{}} % Adjusted for 8 columns of data
    \toprule
    & \multicolumn{2}{c}{Push} & \multicolumn{2}{c}{Lift} & \multicolumn{2}{c}{Can} & \multicolumn{2}{c}{Stack} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    & ours & baseline & ours & baseline & ours & baseline & ours & baseline \\
    \midrule
   Masked & \textbf{100.0 $\pm$ 0.00} & 60.7 $\pm$ 10.6 & \textbf{83.3 $\pm$ 6.60} & 0.0 $\pm$ 0.00 & \textbf{44.7 $\pm$ 8.06} & 19.3 $\pm$ 5.25 & \textbf{34.0 $\pm$ 11.43} & 0.7 $\pm$ 0.94 \\
    Zoom in & \textbf{86.0 $\pm$ 2.83} & 8.7 $\pm$ 4.99 & \textbf{80.7 $\pm$ 5.73} & 5.3 $\pm$ 2.49 & \textbf{89.3 $\pm$ 4.11} & 24.7 $\pm$ 1.89 & \textbf{10.7 $\pm$ 4.11} & 8.0 $\pm$ 1.63 \\
    Blurred & \textbf{80.7 $\pm$ 9.84} & 16.7 $\pm$ 3.77 & \textbf{93.3 $\pm$ 0.94} & 48.0 $\pm$ 5.89 & \textbf{34.7 $\pm$ 4.11} & 2.67 $\pm$ 1.89 & \textbf{62.0 $\pm$ 10.71} & 0.7 $\pm$ 0.94 \\
    Gaussian Noise & \textbf{100.0 $\pm$ 0.00} & 59.3 $\pm$ 6.80 & \textbf{91.3 $\pm$ 5.73} & 9.3 $\pm$ 4.11 & \textbf{30.7 $\pm$ 6.80} & 6.0 $\pm$ 4.32 & \textbf{34.0 $\pm$ 7.12} & 24.0 $\pm$ 2.83 \\
    Camera Type & \textbf{100.0 $\pm$ 0.00} & 29.3 $\pm$ 7.36 & \textbf{79.3 $\pm$ 2.49} & 14.7 $\pm$ 4.99 & \textbf{92.7 $\pm$ 2.50} & 29.3 $\pm$ 3.40 & \textbf{22.7 $\pm$ 3.77} & 0.0 $\pm$ 0.00 \\
    Camera Position & \textbf{100.0 $\pm$ 0.00} & 19.3 $\pm$ 5.73 & \textbf{93.3 $\pm$ 2.49} & 36.0 $\pm$ 1.63 & \textbf{44.7 $\pm$ 3.40} & 1.3 $\pm$ 1.89 & \textbf{26.0 $\pm$ 4.32} & 14.0 $\pm$ 3.27 \\
    \bottomrule
  \end{tabular}
  \caption{\textbf{Zero-Shot Transfer Success Rates in Simulation.} We report the success rates of four manipulation tasks and six different visual modalities. Each mean value and the standard deviation are calculated with three random seeds. Our result shows that PeS constantly outperforms the baseline in all the tasks. It achieves 100\% of success rates in some simple tasks while the baseline has only 20\% to 60\%. In some hard tasks where the baseline success rates are close to 0, PeS can still achieve over 20\% of success rates.}
  \vspace{-10pt} % Adjust the space below the caption
  \label{tab:sim_zero_shot}
\end{table*}
